Tri-Modal Motion Retrieval by Learning a Joint Embedding Space

Information retrieval is an ever-evolving and crucial research domain. The substantial demand for high-quality human motion data especially in online acquirement has led to a surge in human motion research works. Prior works have mainly concentrated on dual-modality learning, such as text and motion tasks, but three-modality learning has been rarely explored. Intuitively, an extra introduced modality can enrich a model's application scenario, and more importantly, an adequate choice of the extra modality can also act as an intermediary and enhance the alignment between the other two disparate modalities. In this work, we introduce LAVIMO (LAnguage-VIdeo-MOtion alignment), a novel framework for three-modality learning integrating human-centric videos as an additional modality, thereby effectively bridging the gap between text and motion. Moreover, our approach leverages a specially designed attention mechanism to foster enhanced alignment and synergistic effects among text, video, and motion modalities. Empirically, our results on the HumanML3D and KIT-ML datasets show that LAVIMO achieves state-of-the-art performance in various motion-related cross-modal retrieval tasks, including text-to-motion, motion-to-text, video-to-motion and motion-to-video.

==> sec/0_abstract.tex <==
\begin{abstract}
Text-to-motion tasks have been the focus of recent advancements in the human motion domain. However, the performance of text-to-motion tasks have not reached its potential, primarily due to the lack of motion datasets and the pronounced gap between the text and motion modalities. To mitigate this challenge, we introduce VLMA, a novel Video-Language-Motion Alignment method. This approach leverages human-centric videos as an intermediary modality, effectively bridging the divide between text and motion. By employing contrastive learning, we construct a cohesive embedding space across the three modalities. Furthermore, we incorporate a motion reconstruction branch, ensuring that the resulting motion remains closely aligned with its original trajectory. Experimental evaluations on the HumanML3D and KIT-ML datasets demonstrate the superiority of our method in comparison to existing approaches. Furthermore, we introduce a novel task termed video-to-motion retrieval, designed to facilitate the seamless extraction of corresponding 3D motions from an RGB video. Supplementary experiments demonstrate that our model is extensible to real-world, human-centric videos, offering a valuable complement to the pose estimation task.
\end{abstract}


==> sec/1_intro.tex <==
\beforesection
\section{Introduction}
\aftersection
\label{sec:intro}
\quad Natural Language Processing (NLP) and generative models such as Generative Adversarial Network (GAN)~\cite{goodfellow2014generative}, diffusion model~\cite{ho2020denoising, ho2022classifier, song2020denoising} and GPT-4~\cite{vaswani2017attention,openai2023gpt4} have made substantial progress. Text as one of the most prevalent and natural modalities in human daily life has captured significant research interest. A growing number of cross-modal tasks related to text, such as text-to-image~\cite{reed2016generative, ramesh2021zero, ding2021cogview, zhang2023controllable}, text-to-video~\cite{balaji2019conditional, ho2022imagen, wu2023cap4video} and text-to-motion~\cite{guo2022tm2t, petrovich2022temos, chen2023executing} have burst onto the academic scene. Owing to the abundance of accessible high quality datasets, text-to-image and text-to-video tasks have achieved considerable success. A large amount of works such as CLIP~\cite{ramesh2021zero}, DALL$\cdot$E 2~\cite{ramesh2022hierarchical}  and Make-A-Video~\cite{singer2022make} can generate high quality images or videos given texts. The concept of text-to-motion entails that, given a textual description, the model can acquire corresponding 3D human motion sequences either by retrieval~\cite{petrovich23tmr} or generation~\cite{guo2022tm2t, tevet2022human, zhang2022motiondiffuse, jiang2023motiongpt}.
Currently, the fidelity of generated motions is hindered partly by the limited availability of comprehensive motion datasets, and by the need for further refinement and enhancement of the models themselves. Motion retrieval, which entails searching for the closest matches within a large motion database, has found widespread application in various industries, such as character animation~\cite{holden2017phase, bergamin2019drecon} and virtual fitting rooms~\cite{han2018viton}. A key benefit of motion retrieval is the elimination of concerns over the authenticity of the resulting motions. This paper focuses on text-to-motion retrieval, a nascent field recently introduced by TMR~\cite{petrovich23tmr}.
However, the expense of motion capture technology required to create motion datasets is exorbitantly high, not to mention the significant costs for manually annotating text descriptions. These factors collectively contribute to the scarcity of motion datasets. Consequently, the quality of retrieved motions significantly lags behind what is currently achievable in the video and image domains.

\begin{figure}
    \centering
\includegraphics[width=\columnwidth]{Picture/method_overview.pdf}
    \caption{\textbf{Overview of VLMA.} During the training phase, each of the three modalities is processed through distinct encoders. Subsequently, the resultant embeddings are aligned within a unified joint embedding space utilizing contrastive learning techniques. In the inference stage, the model is capable of accepting texts or videos as input queries, enabling the retrieval of corresponding motion data effectively.}
    \label{fig:1}
\end{figure}

%1.human-centric video是3Dmotion的低维表示，所以我们提出让human-centric video作为motion-text任务中的一个辅助模态。（这里作为辅助模态的原因仅仅是低维表示嘛？）2. 现在有大量的视频文本的数据集，同时在action recognition任务中，也有许多高质量的human-centric的video action label数据集，用他们训练的模型的知识可以迁移到motion领域来。3. 所以我们的做法是在两个常用的数据集上都增加了video模态，并利用pretrain-model的先验知识来减少模型对motion的依赖。


The spatial distance between text and motion is considerably vast, which poses challenges in effectively merging them into a unified embedding space. In comparison, the human-centric video modality serve as a compact, low-dimensional representation of intricate 3D motions, placing it closer in the spatial spectrum to motion. Concurrently, the availability of numerous video-text datasets especially in the pose estimation field bolsters the integration of the human-centric video and text modalities. Given these factors, we propose video as an apt auxiliary modality to facilitate the alignment training between text and motion. The idea echoes methodologies seen in the video-language comprehension domain, VALOR~\cite{chen2023valor} leverages audio as an auxiliary modality to bolster the alignment between video and language. Building upon the integration of video into our cross-modal learning framework, we not only facilitate text-to-motion retrieval task but also empower our model to execute video-to-motion retrieval task.

We assess our proposed approach using two standard text-to-motion benchmarks: HumanML3D~\cite{Guo_2022_CVPR} and KIT-ML~\cite{Plappert2016}. 
Comprehensive quantitative analysis show that our method surpasses existing text-to-motion retrieval techniques by a notable margin. Meanwhile, we achieve a higher accuracy in video-to-motion retrieval than MotionCLIP~\cite{tevet2022motionclip}. Furthermore, we have extended our framework to encompass real-life, human-centric video content. Through a user study, the results indicate that our model successfully retrieves the correct motion in the majority of cases. 
To the best of our knowledge, this paper first propose to leverage video as an auxiliary modality to amplify the alignment between text and motion.

Our key contributions are summarized as follows. (i) We introduce Video-Language-Motion Alignment (VLMA), a framework designed to cultivate a cohesive embedding space across the three aforementioned modalities. This architecture can accomplish both text-to-motion retrieval and video-to-motion retrieval tasks.
(ii)
(iii) In our efforts to enrich the available data, we have augmented both the HumanML3D and KIT datasets with RGB videos. This was achieved by animating and rendering avatars corresponding to specific motions. Such augmentation paves the way for more expansive and informed multi-modal research in human motion dynamics.\red{need to think of how to summarize technical contributions.}


==> sec/3_method.tex <==
\beforesection
\section{Method}
\aftersection
\quad Our primary goal is to train a joint embedding space of three modalities, \ie text, video and motion, ideally allowing to mutually represent each other. With this embedding space, one can accomplish various tasks involving the retrieval from text to motion or from video to motion. In this section, we begin by providing a comprehensive definition of the three related modalities along with their distinct encoders in Sec.~\ref{sec3.1} Following that, we detail the explanation of the negative filtering and present the three-modality co-training process in Sec.~\ref{sec3.2}. Finally, Sec.~\ref{sec3.3} offers implementation details.
%For a clearer understanding of our task, we present a brief description of the text and motion modalities, as well as the auxiliary video modality. {\bf Motion Sequence} comprises a series of 3D human poses $M_i=[H_1, H_2, ..., H_f]$,\red{$f$ means?} where $f$ represents the total frames of a motion sequence. Each pose is parameterized using the SMPL model~\cite{SMPL:2015}. We follow TMR to employ the motion representation used in~\cite{guo2022generating}, which consists of joint velocities, local joint positions, 6D form local joint rotations and the foot contact label. {\bf Text Description} consists of a series of words $T_i=[W_1, W_2, ..., W_n]$ which concisely summarize motion contents. It often includes elements such as the target character (e.g., 'The man'), the specific actions performed by the character (e.g., 'doing jumping jacks'), and the stylistic attributes that characterize these actions (e.g., 'at a fast speed', 'counterclockwise'). Furthermore, one text description may involve multiple actions combined in a sequence (e.g., 'The man walks forward at a rapid pace and then makes a right turn.').  {\bf RGB Video} can be represented as a number of frames $V_i=[F_1, F_2, ..., F_f]$ \red{what about $V_i\in\mathbb{R}^{N\times H\times W\times 3}$}. Where $F_i$ corresponds to the $i$-th frame in the series. \red{delete this sentence}Throughout the training phase, due to the absence of real-world human-centric RGB videos that are paired with the HumanML3D and KIT-ML datasets, we rendered smpl based on the 3D motion sequences. 
% We randomly extract 8 frames at regular intervals from the video. Take a video of 200 frames for an example, we randomly choose an integer $x$ such that $x \in \{0, 1, \ldots, 25\}$, the sampled video frames are: $x + \{0, 25, 50, 75, 100, 125, 150, 175\}$.
%We uniformly sample $N$ frames from an RGB video as the input to avoid redundancy.
%\red{mention the value of N and how to augment input video in implementation details}
% Utilizing this sampling technique allows us to sample nearly all video frames during the training process. Also we can ensure that the 8 sampled frames can represent the corresponding motions only with a low FPS.

\subsection{Modality Definitions and Model Architecture}
\label{sec3.1}
\quad Our comprehensive model architecture comprises a motion encoder, a text encoder, and a video encoder. 
Motion, text, and video features are extracted individually through their respective encoders and then aligned within the joint embedding space. To expedite convergence, we initialized our model parameters using pre-trained models.

{\bf Motion Encoder}. The Motion Sequence comprises a series of 3D human poses $P=[P_1, P_2, ..., P_{S_m}]$, where $S_m$ represents the temporal length of a motion sequence. Each pose is parameterized using the SMPL model~\cite{SMPL:2015}. We follow TMR to employ the motion representation used in~\cite{guo2022generating}, which consists of joint velocities, local joint positions, 6D form local joint rotations and the foot contact label. We utilize the motion encoder from MotionCLIP~\cite{tevet2022motionclip} in our work. 
The motion sequences are denoted as $P \in {\mathbb{R}}^{S_m \times C_m}$, where $S_m$ is the sequence length, $C_m$ is the feature of a single pose. The sequences undergo a linear projection, mapping them into the latent dimension. Subsequently, a [CLS] token, representing the global feature of the motion sequence is appended at the beginning of the entire sequence. The processed sequence is then fed into a transformer encoder. We select the first position of the output as the representative motion feature, denoted as $e_m\in \mathbb{R}^{C}$, where $C$ is the latent dimension.

{\bf Text Encoder} Text Description consists of a series of words $T=[W_1, W_2, ..., W_n]$ which concisely summarize motion contents. It often includes elements such as the target character (e.g., 'The man'), the specific actions performed by the character (e.g., 'doing jumping jacks'), and the stylistic attributes that characterize these actions (e.g., 'at a fast speed', 'counterclockwise'). Furthermore, one text description may involve multiple actions combined in a sequence (e.g., 'The man walks forward at a rapid pace and then makes a right turn.'). We employ DistilBERT~\cite{DBLP:journals/corr/abs-1910-01108} as the foundational model. Textual tokens are generated through the DistilBERT tokenizer. Following the architecture of the motion encoder, a [CLS] token is appended to the start of the token sequence. This complete sequence is subsequently fed into the transformer encoder. The textual feature representation is extracted from the first output position, denoted as $e_t\in \mathbb{R}^{C}$, where $C$ is the latent dimension.

{\bf Video Encoder}.  RGB Video can be represented as a number of frames $V_i\in\mathbb{R}^{S_v\times H\times W\times 3}$. 
% Throughout the training phase, due to the absence of real-world human-centric RGB videos that are paired with the HumanML3D and KIT-ML datasets, we rendered smpl based on the 3D motion sequences. 
We uniformly sample $S_v$ frames from an RGB video as the input to avoid redundancy. The video encoder consists of a CLIP image encoder and a temporal transformer. 
% The video sequences are represented as $V_i \in {\mathbb{R}}^{S_v \times C \times H \times W}$, where $S_v$ denotes the selected frames of a video, $C$ represents the channel size, and $H$ and $W$ are the height and width of each video frame respectively. 
Initially, we pass the video sequences through the CLIP pre-trained image encoder to obtain the image features corresponding to each selected frame. Subsequently, taking into account the temporal aspects of the video, we input these image features into a temporal transformer. The video embedding is obtained by applying average pooling to the output of the temporal transformer, denoted as $e_v\in \mathbb{R}^{C}$, where $C$ is the latent dimension.


\subsection{Cross-Modality Contrastive Learning}
\label{sec3.2}
\quad {\bf Multi-Modality Alignment}. We employ contrastive learning to construct a fine-grained embedding space that bridges the three modalities. 
Initially, we designate $S_{target}$ as the target similarity matrix. 
Given the reality that various text descriptions might convey analogous meanings, defining $S_{target}$ solely as an identity matrix can be problematic. 
This would lead the model to treat texts with similar implications as negative pairs, hampering optimal performance in the text-motion retrieval task. 
To address the aforementioned issue, we adopt the negative filtering technique as proposed by TMR~\cite{petrovich23tmr}. 
%Specifically, we utilize a pre-trained language model to encode texts into embeddings, denoted as $T_e$. 
Subsequently, we compute the cosine similarity between pairs of text embeddings within a single batch of size $B$. 
A threshold $\epsilon$ is defined to represent the minimum similarity score acceptable for a pair to be considered positive. 
Contrary to the approach in TMR, instead of merely discarding scores above the threshold $\epsilon$, we retain them in $S_{target}$. 
%Our ablation studies indicate that preserving these high-similarity pairs contributes to improved retrieval performance. 
% So, the formula for the target similarity matrix can be written as follows.
So we have the target similarity matrix $S_{target}\in\mathbb{R}^{B\times B}$ with its element defined as\red{Kangning: Here, $e_t$ is not the output of distilbert, it is computed by a pre-trained language model, so can we write $e_t$ here?}
\begin{equation}
    S_{target}(i,j) = 
    \left\{
        \begin{aligned}
        & cos(e_{t}^{i}, e_{t}^{j}), & \text{if }  cos(e_{t}^{i}, e_{t}^{j}) \ge \epsilon, \\
        & 0, & \text{otherwise}.
        \end{aligned}
    \right.
\end{equation}
$cos(\cdot)$ is the consine similarity between the input two embeddings, defined as:
\begin{equation}
    cos(e_{t}^{i}, e_{t}^{j})= \frac{ e_{t}^{i} \cdot e_{t}^{j\top} }{ \lVert e_{t}^{i} \rVert \lVert e_{t}^{j} \rVert }
\end{equation}
Take text and motion modalities for an example, the similarity matrix between text to motion and motion to text can be calculated as follows: 
% \red{what is X and Y? can write "between two modalities. For example, we have the similarity matrix between text and motion denoted as ${S_{pred}^{t,m}}$"}
% Subsequently, we compute the softmax similarity scores, denoted as ${S_{pred}^{XY}}$, between the embeddings of modality X and modality Y.
\begin{equation}
S_{pred}^{t2m}(i) = \frac{\exp(cos({\bm{e_{t}}}, e_{m}^i)/ \tau)}{\sum_{j=1}^{B} \exp(cos({\bm e_{t}}, e_{m}^j)/ \tau)}
\end{equation}
\begin{equation}
S_{pred}^{m2t}(i) = \frac{\exp(cos({\bm e_{m}}, e_{t}^i)/ \tau)}{\sum_{j=1}^{B} \exp(cos({\bm e_{m}}, e_{t}^j)/ \tau)}
\end{equation}
where $\tau$ is the learnable temperature parameter. To maximize the proximity between positive samples while increasing the distance between negative samples, we employ the Kullback–Leibler (KL) divergence loss to optimize our joint embedding space between text and motion
\begin{equation}
\mathcal{L}_{align}^{mt} = KL\left({S_{pred}^{t2m}}, {S_{target}}
\right)+KL\left({S_{pred}^{m2t}}, {{S_{target}}^T}\right)
\end{equation}
Thus, the comprehensive alignment loss is computed as the aggregate of the alignment losses across the three modalities.
\begin{equation}
    \mathcal{L}_{align} = \mathcal{L}_{align}^{mt} + \mathcal{L}_{align}^{mv} + \mathcal{L}_{align}^{tv}
\end{equation}

\begin{figure}
    \centering
\includegraphics[width=\columnwidth]{Picture/feature_fusion.pdf}
    \caption{caption}
    \label{fig:2}
\end{figure}

\quad {\bf Feature Fusion}. 
Contemporary multi-modal alignment methodologies invariably integrate a reconstruction branch to ensure that the representations learned are faithful to the original input data. However, such approaches typically concentrate solely on the modality being reconstructed, thus neglecting the potential insights offered by additional modalities. Inspired by the query, key and value framework prevalent in natural language processing literature~\cite{wang2019coke, gao2022calic}, we tailor this paradigm to address the intricacies of modality alignment. 
\red{this sentence can move to the place after describing how to do. The logic is first describe how to do this, then explain why to do this.}Through the application of self-attention mechanism, we can effectively absorb and fuse the most relevant features from other modalities, thereby enhancing the precision of motion reconstruction and the alignment of the three modalities. 

%Current multi-modal alignment always incorporate a reconstruction branch to ensure that the learned representations maintain fidelity to the original input data. However, it only foucs on the reconstructed modality itself, overlooking other modalities that may contain useful information. To addressing this issue, we introduce a specially designed attention mechanism into the reconstruction branch to enhance the alignment among text, video, and motion modalities. By doing this, our framework not only focuses on the explicit alignment across modalities but also delves into their latent, more implicit correlations through the attention mechanism, achieving a finer integration of information. Drawing inspiration from the Query, Key, Value paradigm in natural language processing~\cite{wang2019coke, gao2022calic}, we adapt this concept to the challenge of modality alignment. Self-attention can effectively weigh the importance of different features from each modality, learning to highlight crucial aspects that contribute to a more accurate reconstruction of motion. The attention mechanism can be written as: 



As text may convey subtle details not readily apparent in motions or videos, such as intentions, explicit actions, or temporal nuances ("quickly" or "slowly"), it holds unique value. Similarly, videos provide visual context that may not be captured by text or motion. By absorbing information from text and video modalities, our model is able to resolve the ambiguities and fill in the informational voids within the motion modality. Therefore, we treat motion embeddings as queries that actively seek out and engage with relevant information across both textual and visual domains. The process can be written as:

\begin{footnotesize}
    \begin{equation}
    \Tilde{e}_m=Atten(e_m, e_m, e_m) + Atten(e_m, e_t, e_t) + Atten(e_m, e_v, e_v),
    \end{equation}
\end{footnotesize}
where $Atten$ means self-attention operations proposed in~\cite{vaswani2017attention}. 
Then the fused embedding $\Tilde{e}_m$ is then fed into the motion decoder, whose role is to reconstruct the motion sequences, denoted as $M_{recon}$. To quantify the discrepancy between the original and reconstructed motions, we employ a Mean Squared Error (MSE) loss function.
\begin{equation}
    \mathcal{L}_{recon} = MSE(M, M_{recon})
\end{equation}
Finally, our whole loss function as be formulated as:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{align} + {\lambda}_{recon} \cdot \mathcal{L}_{recon}
\end{equation}
Where ${\lambda}_{recon}$ is the weight of the reconstruction loss, we set it to 0.1 during our training process.


% {\bf Motion Decoder}. For Motion Decoder, We follow that of MotionCLIP~\cite{tevet2022motionclip} and TEMOS~\cite{petrovich2022temos}. We feed a latent motion representation $z$ along with the duration of the motion sequence $T$ into a transformer decoder to acquire the reconstructed motion sequence, denoted as $M_{recon}$.

%By processing text, video, and motion data as a sequential input into our Transformer encoder, our model leverages the internal self-attention mechanism to learn the intrinsic connections between different modalities. This approach not only improves the interoperability between modalities but also enables the motion modality to integrate features from text and video more richly. This central contribution represents the core innovation of our work, offering a novel perspective for multimodal learning and paving the way for future research.
%To optimally harness both text and video data for enriching motion representation, we introduce the feature fusion module. Specifically, we organize the embeddings of the three modalities into a sequential format, spanning a length of three, which is subsequently fed into a transformer. The output derived from the transformer encoder is employed to reconstruct the motion sequence. Our primary aim is to utilize the attention mechanism to integrate information from these three modalities, meanwhile ensuring that the integrity of the original motion embedding is preserved to the greatest extent possible.


==> sec/Chart.tex <==
\section{Chart}
\begin{table*}
    \centering
    \caption{HumanML3D}
    \small
    \setlength{\tabcolsep}{1.0pt}
    \begin{tabular}{l|l|*{6}{>{\centering\arraybackslash}m{1.0cm}}|*{6}{>{\centering\arraybackslash}m{1.0cm}}}
        \toprule
        \textbf{Protocol} & \textbf{Methods} & \multicolumn{6}{c|}{\textbf{Text-motion retrieval}} & \multicolumn{6}{c}{\textbf{Motion-text retrieval}} \\
        & & R@1↑ & R@2↑ & R@3↑ & R@5↑ & R@10↑ & MedR↓ & R@1↑ &R@2↑ & R@3↑ & R@5↑ & R@10↑ & MedR↓ \\
        \midrule
        (a) All & TEMOS ~\cite{petrovich2022temos} & 2.12 & 4.09 & 5.87 & 8.26 & 13.52 & 173.0 & 3.86 & 4.54 & 6.94 & 9.38 & 14.00& 183.25 \\
        & Guo et al. ~\cite{Guo_2022_CVPR} & 1.80 & 3.42 & 4.79 & 7.12 & 12.47 & 81.0 &  2.92 & 3.74 & 6.00 & 8.36 & 12.95 & 81.50 \\
        & TMR~\cite{petrovich23tmr} & 5.68 & 10.59 & 14.04 & 20.34 & 30.94 & 28.00 &  9.95 & 12.44 & 17.95 & 23.56 & 32.69 &28.50 \\
        &Ours(2Modal) & 5.93 & 10.89 & 14.67 & 20.78 & 32.47 & \bf24.00 & 8.08 & 12.30 &   16.85 & 23.39 & 34.64 & 23.50 \\
        & Ours(3Modal) & \bf6.37 & \bf11.84 & \bf15.60 & \bf21.95 & \bf33.67 & \bf24.00 & \bf9.72 & \bf13.33 & \bf18.73 & \bf25.00 & \bf36.55 & \bf22.50 \\
        \midrule
        (b) All with threshold & TEMOS ~\cite{petrovich2022temos} & 5.21 & 8.22 & 11.14 & 15.09 & 22.12 & 79.00 &  5.48 & 6.19 & 9.00 & 12.01 & 17.10 &129.0 \\
        & Guo et al. ~\cite{Guo_2022_CVPR} & 5.30 & 7.83 & 10.75 & 14.59 & 22.51 & 54.00 & 4.95 & 5.68 & 8.93 & 11.64 & 16.94 &69.50\\
        & TMR~\cite{petrovich23tmr} & 11.60 & 15.39 & 20.50 & 27.72 & 38.52 & 19.00 & 13.20 & 15.73 & 22.03 & 27.65 & 37.63 & 21.50 \\
        &Ours(2Modal) & 11.32 & 15.01 & 20.91 & 27.93 & 40.97 & 17.00 & 12.95 & \bf17.56 & 22.69 & 29.05 & 39.58 & 19.00 \\
        & Ours(3Modal) & \bf12.94 & \bf17.38 & \bf23.63 & \bf30.13 & \bf42.46 & \bf16.00 & \bf13.89 & 17.11 & \bf23.83 & \bf29.93 & \bf41.09 & \bf17.50\\
        \midrule
        (c) Dissimilar subset & TEMOS ~\cite{petrovich2022temos} & 20.00 & 33.00 & 37.00 & 47.00 & 62.00 & 6.00 & 24.00 & 30.00 & 39,00 & 47.00 & 62.00 & 6.74 \\
        & Guo et al. ~\cite{Guo_2022_CVPR} & 13.00 & 27.00 & 39.00 & 51.00 & 72.00 & 5.00 & 24.00 & 39.00 & 46.00 & 58.00 & 71.00 & 4.50 \\
        & TMR~\cite{petrovich23tmr} & 34.00 & 56.00 & 61.00 & 68.00 & 76.00 & 2.00 & 47.00 & 55.00 & 65.00 & 71.00 & 78.00 & 2.50 \\
        & Ours(2Modal) & \bf51.00 & 63.00 & 69.00 & 76.00 & 80.00 & 1.50 & 52.00 & 65.00 & 70.00 & 77.00 & 80.00 & \bf1.00 \\
        &Ours(3Modal) & 50.00 & \bf71.00 & \bf79.00 & \bf86.00 & \bf90.00 & \bf1.00 & \bf56.00 & \bf73.00 & \bf81.00 & \bf86.00 & \bf92.00 & \bf1.00 \\
        \midrule
        (d) Small batches ~\cite{Guo_2022_CVPR} & TEMOS ~\cite{petrovich2022temos} & 40.49 & 53.52 & 61.14 & 70.96 & 84.15 & 2.33 & 39.96 & 53.49 & 61.79 & 72.40 & 85.89 & 2.33 \\
        & Guo et al. ~\cite{Guo_2022_CVPR} & 52.48 & 71.05 & 80.65 & 89.86 & 96.58 & 1.39 & 52.00 & 71.21 & 81.11 & 89,87 & 96.78 & 1.38 \\
        &TMR~\cite{petrovich23tmr} & 67.16 & 81.32 & 86.81 & 91.43 & 95.36 & 1.04 & 67.97 & 81.20 & 86.35 & 91.70 & 95.27 & 1.03  \\
        &Ours(2Modal) & 66.74 & 78.98 & 83.67 & 87.29 & 91.66 & 1.02 & 67.87 & 79.62 & 84.08 & 88.27 & 91.61 & \bf1.01 \\
        &Ours(3Modal) & \bf68.58 & \bf81.04 &\bf85.02 & \bf88.77 & \bf92.58 & \bf1.01 & \bf68.64 & \bf81.06 & \bf85.52 & \bf88.76 & \bf92.82 & \bf1.01 \\
        % ... 接下来的行与上面的类似，填写相应的数据 ...
    \bottomrule
    \end{tabular}
\end{table*}
\label{table1}

\begin{table*}
    \centering
    \caption{KIT-ML}
    \small
    \setlength{\tabcolsep}{1.0pt}
    \begin{tabular}{l|l|*{6}{>{\centering\arraybackslash}m{1.0cm}}|*{6}{>{\centering\arraybackslash}m{1.0cm}}}
        \toprule
        \textbf{Protocol} & \textbf{Methods} & \multicolumn{6}{c|}{\textbf{Text-motion retrieval}} & \multicolumn{6}{c}{\textbf{Motion-text retrieval}} \\
        & & R@1↑ & R@2↑ & R@3↑ & R@5↑ & R@10↑ & MedR↓ & R@1↑ &R@2↑ & R@3↑ & R@5↑ & R@10↑ & MedR↓ \\
        \midrule
        (a) All & TEMOS ~\cite{petrovich2022temos} & 7.11 & 13.25 & 17.59 & 24.10 & 35.66 & 24.00 & 11.69 & 15.30 & 20.12 & 26.63 & 36.39 & 26.50 \\
        & Guo et al. ~\cite{Guo_2022_CVPR} & 3.37 & 6.99 & 10.84 & 16.87 & 27.71 & 28.00 & 4.94 & 6.51 & 10.72 & 16.14 & 25.30 & 28.50 \\
        & TMR~\cite{petrovich23tmr} & 7.23 & 13.98 & 20.36 & 28.31 & 40.12 & 17.00 &  11.20 & 13.86 & 20.12 & 28.07 & 38.55 & 18.00 \\
        &Ours(2-modal) & 8.59 & 15.04 & 21.09 & 32.23 & 46.09 & 13.00 & 11.72 & 17.19 & 23.63 & 32.81 & 48.83 & 12.00 \\
        %&Ours(normal) & {\bf 11.33} & 19.14 & 24.21 & 34.18 & 46.68 & {\bf11.00} & 14.65 & {\bf20.90} & \bf 27.34 & \bf 36.13 & 50.39 & 11.50 \\
        &Ours(3-modal) & \bf10.16 & {\bf 19.92 } & {\bf24.61} & {\bf34.57} & {\bf49.80} & {\bf11.00} & {\bf15.43} & \bf20.12 & \bf26.95 & \bf34.57 & \bf53.32 & \bf10.00 \\
        \midrule
        (b) All with threshold & TEMOS ~\cite{petrovich2022temos} & 18.55 & 24.34 & 30.84 & 42.29 & 56.37 & 7.00 &  17.71 & 22.41 & 28.80 & 35.42 & 47.11 & 13.25 \\
        & Guo et al. ~\cite{Guo_2022_CVPR} & 13.25 & 22.65 & 29.76 & 39.04 & 49.52 & 11.00 & 10.48 & 13.98 & 20.48 & 27.95 & 38.55 & 17.25\\
        & TMR~\cite{petrovich23tmr} & 24.58 & 30.24 & 41.93 & 50.48 & 60.36 & 5.00 & 19.64 & 23.73 & 32.53 & 41.20 & 53.01 & 9.50 \\
        &Ours(2-modal) & 24.02 & 30.86 & 42.73 & 54.69 & 70.09 & 5.0 & 21.68 & 27.93 & 34.18 & 42.77 & 57.42 & 8.0\\
        %&Ours(normal) & 25.22 & 35.73 & 45.82 & 57.20 & 68.88 & \bf4.00 & 24.06 & 29.39 & 36.46 & 45.53 & 56.63 & 8.00 \\
        &Ours(3-modal) & \bf30.86 & \bf41.80 & \bf48.63 & \bf59.96 & \bf74.22 & \bf4.00 & \bf25.98 & \bf31.25 & \bf38.28 & \bf45.70 & \bf63.09 & \bf6.50 \\
        \midrule
        (c) Dissimilar subset & TEMOS ~\cite{petrovich2022temos} & 24.00 & 40.00 & 46.00 & 54.00 & 70.00 & 5.00 & 33.00 & 39.00 & 45.00 & 49.00 & 64.00 & 6.50 \\
        & Guo et al. ~\cite{Guo_2022_CVPR}] & 16.00 & 29.00 & 36.00 & 48.00 & 66.00 & 6.00 & 24.00 & 29.00 & 36.00 & 46.00 & 66.00 & 7.00 \\
        & TMR~\cite{petrovich23tmr} & 26.00 & 46.00 & 60.00 & 70.00 & 83.00 & 3.00 & 34.00 & 45.00 & 60.00 & 69.00 & 82.00 & 3.50 \\
        &Ours(2-modal) & 29.00 & 45.00 & 60.00 & 71.00 & 81.00 & 2.00 & 43.00 & 59.00 & 67.00 & 73.00 & \bf83.00 &2.00 \\
        %&Ours(normal) & \bf35.00 & \bf52.00 & \bf64.00 & \bf78.00 & \bf87.00 & \bf2.00 & 41.00 & 55.00 & 69.00 & 75.00 & \bf86.00 & \bf2.00 \\
        &Ours(3-modal) & \bf30.00 & \bf49.00 & \bf63.00 & \bf73.00 & \bf84.00 & \bf3.00 & \bf48.00 & \bf60.00 & \bf66.00 & \bf76.00 & 82.00 & \bf2.00 \\
        \midrule
        (d) Small batches ~\cite{Guo_2022_CVPR} & TEMOS ~\cite{petrovich2022temos} & 43.88 & 58.25 & 67.00 & 74.00 & 84.75 & 2.06 & 41.88 & 55.88 & 65.62 & 75.25 & 85.75 & 2.25 \\
        & Guo et al. ~\cite{Guo_2022_CVPR} & 42.25 & 62.62 & 75.12 & 87.50 & 96.12 & 1.88 & 39.75 & 62.75 & 73.62 & 86.88 & 95.88 & 1.95 \\
        &TMR~\cite{petrovich23tmr} & 49.25 & 69.75 & 78.25 & 87.88 & 95.00 & 1.50 & 50.12 & 67.12 & 76.88 & 88.88 & 94.75 & 1.53  \\
        &Ours(2-modal) & 53.96 & 76.42 & 82.05 & 89.66 & 95.22 & 1.38 & 58.58 & 75.05 & 81.84 & 89.68 & 93.86 &1.23 \\
        %&Ours(normal) & \bf58.76 & 76.79 & 83.77 & 91.72 & 94.71 & 1.21 & 58.20 & 74.79 & 83.86 & 91.60 & 94.88 & 1.21 \\
        &Ours(3-modal) & \bf58.10 & \bf77.80 & \bf86.34 & \bf93.08 & \bf96.47 & \bf1.08 & \bf60.23 & \bf77.52 & \bf86.44 & \bf93.22 & \bf95.87 & \bf1.20 \\
        % ... 接下来的行与上面的类似，填写相应的数据 ...
    \bottomrule
    \end{tabular}
\end{table*}
\label{table2}

\begin{table*}
    \centering
    \caption{HumanML3D}
    \small
    \setlength{\tabcolsep}{1.0pt}
    \begin{tabular}{l|l|*{6}{>{\centering\arraybackslash}m{1.0cm}}|*{6}{>{\centering\arraybackslash}m{1.0cm}}}
        \toprule
        \textbf{Protocol} & \textbf{Methods} & \multicolumn{6}{c|}{\textbf{Video-motion retrieval}} & \multicolumn{6}{c}{\textbf{Motion-video retrieval}} \\
        & & R@1↑ & R@2↑ & R@3↑ & R@5↑ & R@10↑ & MedR↓ & R@1↑ &R@2↑ & R@3↑ & R@5↑ & R@10↑ & MedR↓ \\
        \midrule
        (a) All & MotionCLIP ~\cite{tevet2022motionclip} & 4.96 & 9.40 & 12.48 & 17.46 & 26.46 & 43.00 & 3.52 & 7.28 & 9.74 & 13.82 & 22.34 & 58.00\\
        &Ours(3-modal) & \bf21.25 & \bf41.38 & \bf50.51 & \bf63.40 & \bf77.50 & \bf3.00 & \bf25.76 & \bf45.36 & \bf54.71 & \bf66.87 & \bf79.73 & \bf3.00\\
        \midrule
        (b) All with threshold & MotionCLIP ~\cite{tevet2022motionclip} & 7.10 & 12.62 & 16.67 & 22.56 & 32.23 & 29.00 & 5.71 & 9.20 & 12.35 & 17.41 & 28.0 &38.00\\
        &Ours(3-modal) & \bf30.42 & \bf46.97 & \bf56.82 & \bf68.77 & \bf81.41 & \bf3.00 & \bf35.43 & \bf52.73 & \bf61.93 & \bf72.95 & \bf84.54 &\bf2.00\\
        \midrule
        (C)Dissimilar subset & MotionCLIP ~\cite{tevet2022motionclip} & 42.00 & 61.00 & 72.00 & 80.00 & 88.00 & 2.00 & 43.00 & 65.00 & 69.00 & 76.00 & 86.00 &2.00\\
        &Ours(3-modal) & \bf74.00 & \bf93.00 & \bf98.00 & \bf100.00 & \bf100.00 & \bf1.00 & \bf79.00 & \bf99.00 & \bf100.00 & \bf100.00 & \bf100.00 &\bf1.00\\
    \bottomrule
    \end{tabular}
\end{table*}
\label{table3}


\begin{table*}
    \centering
    \caption{KIT-ML}
    \small
    \setlength{\tabcolsep}{1.0pt}
    \begin{tabular}{l|l|*{6}{>{\centering\arraybackslash}m{1.0cm}}|*{6}{>{\centering\arraybackslash}m{1.0cm}}}
        \toprule
        \textbf{Protocol} & \textbf{Methods} & \multicolumn{6}{c|}{\textbf{Video-motion retrieval}} & \multicolumn{6}{c}{\textbf{Motion-video retrieval}} \\
        & & R@1↑ & R@2↑ & R@3↑ & R@5↑ & R@10↑ & MedR↓ & R@1↑ &R@2↑ & R@3↑ & R@5↑ & R@10↑ & MedR↓ \\
        \midrule
        (a) All & MotionCLIP ~\cite{tevet2022motionclip} & 3.71 & 6.45 & 8.79 & 11.52 & 17.97 & 52.50 & 4.49 & 7.23 & 9.96 & 12.11 & 21.68 & 51.00\\
        &Ours(3-modal) & \bf18.75 & \bf35.16 & \bf42.58 & \bf55.86 & \bf73.24 & \bf4.00 & \bf23.05 & \bf35.55 & \bf44.14 & \bf56.25 & \bf72.07 & \bf4.00\\
        \midrule
        (b) All with threshold & MotionCLIP ~\cite{tevet2022motionclip} & 8.98 & 12.11 & 14.84 & 19.53 & 27.73 & 27.00 & 9.18 & 12.50 & 17.19 & 22.27 & 33.98 & 21.00\\
        &Ours(3-modal) & \bf36.91 & \bf49.80 & \bf60.94 & \bf70.70 & \bf84.57 & \bf3.00 & \bf41.41 & \bf52.73 & \bf63.28 & \bf75.98 & \bf86.13 & \bf2.00\\
        \midrule
        (C)Dissimilar subset & MotionCLIP ~\cite{tevet2022motionclip} & 15.00 & 23.00 & 31.00 & 40.00 & 59.00 & 8.00 & 13.00 & 21.00 & 25.00 & 41.00 & 63.00 & 6.00\\
        &Ours(3-modal) & \bf66.00 & \bf84.00 & \bf90.00 & \bf96.00 & \bf99.00 & \bf1.00 & \bf66.00 & \bf87.00 & \bf93.00 & \bf98.00 & \bf100.00 & \bf1.00\\
    \bottomrule
    \end{tabular}
\end{table*}
\label{table4}


==> sec/outline.tex <==
\section{outline}
\subsection{introduction}

\subsubsection{text2motion current development, its applications}
give a short overview of the current development of text2motion tasks, especially foucsing on the applications and its challenging

\subsubsection{current text2motion task framework}
current text2motion task framework can be separated into 2 categories. The first is the so called end-to-end framework like MDM. The second is the so called twin tower framework like TEMOS. give a brief description of the two framework mentioned above.
Also, demonstrate the shortcomings of the methods mentioned above

\subsubsection{introduce the multi-modal learning and our method}
give a short overview of the multi-modal learning, remember to mention the VALOR here. 
Previous methods mainly focus on the text2motion task without considering more modalities. The most recent work, MotionCLIP, only considers a static RGB image as an extra modality, neglecting the video-level description of motion dynamics. The necessity of add video modality to the framework?(how to form a good story, add QKV trick here ?)

\subsubsection{our dataset}
We use the HumanML3D and KIT, which are commonly used in recent text to motion works. Furthermore, we extend the two datasets with RGB videos by animating and rendering avatars given a specific motion

\subsubsection{our contributions}
1. Previous methods mainly focus on the text2motion task without considering more modalities. The most recent work, MotionCLIP, only considers a static RGB image as an extra modality, neglecting the video-level description of motion dynamics. We consider multi-modal learning from text, video and motion in an end-to-end framework. 
2. We propose VLMA(Video Language Motion Alignment) to learn a joint embedding space of these three modalities. Our framework is capable of text to motion generation, retrieval, xxx(think of other task, that can not be done by previously methods)
3. We extend HumanML3D KIT datasets with RGB videos by animating and rendering avatars given a specific motion. Our augmentation will definitely promote the future research in multi-modality learning in the area of human motion.

\subsection{Methods}
\subsubsection{Overview}
%Our goal is to build a perfect aligned joint embedding space, where t2m retrieval/generation can all achieve a better performance. Our methods mainly includes three contrastive learning of different modalities. include two modules, cross-modal alignment and conditioned(motion and text) motion reconstruction.
Our goal is to ... Figure1 shows our whole pipeline for... Here make a brief description of our whole pipeline. 
In the following, we first detail the definition of our tasks and the related three modalities in sec 3.1. the specific encoders for the three modalities and their co-training process will be illustrated in sec 3.2. We then make a detailed description of the negative filter and the different modality feature fusion module in sec 3.3. Finally a implementation detail will be give in sec 3.4.
\subsubsection{Definition}
the definition of text description, video frame and 3D motion
\subsubsection{three-modality joint embedding alignment}
Tri-encoder, tell the detail of motion encoder(follow the motionclip), text encoder(TEMOS, but modify the VAE to AE), video encoder(actionclip), our new negative filter trick, which is different from TMR. 
\subsubsection{Attention Module}
make a detail description of how we utilze text information and video information to better construct a motion feature.
\subsubsection{Implementation Detail}


%Model fusion outline
1. 首先我们要达到的一个目的是想通过这个reconstruction loss让motion text video三模态更好的对齐。
2. 实际上模态对齐和Query，Key，Value取回的思想是比较相似的。模态对齐的最终效果其实就是想让各个模态能相互表示，也就是说取回的准确率越高，模态对齐的越好。
3. 所以这里我们就想能不能再reconstruction的过程中，让motion更多的包含上text和video的信息？
4. 想到这里，我们就把text video motion三模态当作了一个sequence length为的sequence，输入到transformer encoder中，利用transformer内部的self-attention机制把这三个模态联系起来
